POI Alias Discovery in Delivery Addresses using User Locations

People often refer to a place of interest (POI) by an alias. In e-commerce scenarios, the POI alias problem affects the quality of the delivery address of online orders, bringing substantial challenges to intelligent logistics systems and market decision-making. Labeling the aliases of POIs involves heavy human labor, which is inefficient and expensive. Inspired by the observation that the users' GPS locations are highly related to their delivery address, we propose a ubiquitous alias discovery framework. Firstly, for each POI name in delivery addresses, the location data of its associated users, namely Mobility Profile are extracted. Then, we identify the alias relationship by modeling the similarity of mobility profiles. Comprehensive experiments on the large-scale location data and delivery address data from JD logistics validate the effectiveness.

==> preproc.tex <==
\section{Pre-Processing}

In the real-world delivery text dataset, due to the mistypes or different writing behavior, there exist many near-duplicate versions of the same POI name/alias. As these near-duplicate aliases essentially refer to the same alias and they are quite similar to each other, putting all of them to the alias list is not only redundant but also very noisy. Moreover, the near-duplicate aliases hinder the performance of mobility profile based solution, as it introduces the \textit{sparsity problem}: Very few people could write exactly the same abnormal address, i.e. such addresses usually associate with only a few users, which causes the mobility profile under-representative. 

By applying the two processes above(i.e. Text Cleaning \& Iterative Clustering), the number of unique aliases is reduced by a lot. For example, in Huqiu District, Suzhou, the number of unique aliases is reduced from over $10,000$ to about only $500$. 



